Centrality Graph Shift Operators for Graph Neural Networks

Graph Shift Operators (GSOs), such as the adjacency and graph Laplacian matrices, play a fundamental role in graph theory and graph representation learning. Traditional GSOs are typically constructed by normalizing the adjacency matrix by the degree matrix, a local centrality metric. In this work, we instead propose and study Centrality GSOs (CGSOs), which normalize adjacency matrices by global centrality metrics such as the PageRank, $k$-core or count of fixed length walks. We study spectral properties of the CGSOs, allowing us to get an understanding of their action on graph signals. We confirm this understanding by defining and running the spectral clustering algorithm based on different CGSOs on several synthetic and real-world datasets. We furthermore outline how our CGSO can act as the message passing operator in any Graph Neural Network and in particular demonstrate strong performance of a variant of the Graph Convolutional Network and Graph Attention Network using our CGSOs on several real-world benchmark datasets.

==> Content/limitations.tex <==
As for the limitations of our approach, rather trivially, the inclusion of centrality metrics is only beneficial if centrality metrics are related to our currently performed learning task on a given dataset. In our experiments, we often observe this case. But this will not hold for all learning tasks and datasets. As a future work, we aim to test the performance of CGNNs on other graph tasks, e.g., link prediction, and to more carefully analyse the learned CGSO parameters. We also aim to extend our theoretical understanding of the CGSOs via further spectral study.  


==> Content/related_work.tex <==

%GSO


% %Centrality
% In parallel, centrality metrics have proved to be insightful in the study of graph theory. Metrics such as degree centrality, closeness centrality, and betweenness centrality have proven to be impactful in revealing key structural properties of graphs \cite{freeman1977set,zhang2017degree}. For instance, the success of PageRank in web links is an illustration of how centrality metrics can reveal the significance and influence of nodes within networks \cite{brin1998anatomy}. Despite their success, the existing GSOs predominantly rely on the simplistic degree normalization, overlooking the potential benefits of leveraging diverse centrality metrics in shaping the operators. While traditional GSOs are often based on degree normalization, the field of Graph Signal Processing (GSP) allows for a broader exploration of normalization strategies, enabling the incorporation of various centrality metrics. This extension opens avenues for enriching GSOs with more nuanced information about the structural importance of nodes in a graph. 

%GNN



%GNN&GSO
% In the context of Graph Neural Networks (GNNs),  GSOs play a pivotal role in capturing the local graph structure. They effectively model the inherent relationships and dependencies among nodes, providing GNN models with the ability to comprehend the flow of information throughout the network. An illustrative example of a GNN architecture leveraging GSOs is the Graph Convolutional Network (GCN) \cite{kipf2016semi}. In GCN, the GSO serves a critical function by influencing the determination of weights that dictate how features from neighboring nodes are amalgamated to update the representation of the target node.


%GSO
% Many common GSOs are often based on normalizing the adjacency matrix using local centrality metrics, such as the degree of nodes \cite{cvetkovic2009towards,xu2018how,kipf2016semi}. GSOs based on degree normalization are effective at capturing local information, and this can make GNNs suitable for tasks that rely on local connectivity. However, while GSOs based on degree normalization have these advantages, they may not be suitable for some settings, especially when non-local information needs to be considered. In this work, we empirically show the limitations of classical GSOs. We also propose \textit{GS-GSO}, new learnable Graph Shift Operators based on global centrality metrics, such as PageRank score, $k$-core number, and the number of walks of a fixed length. 


% Many prevalent Graph Shift Operators (GSOs) often derive from normalizing the adjacency matrix using local centrality metrics, with the degree of nodes being a common choice \cite{cvetkovic2009towards, xu2018how, kipf2016semi}. GSOs employing degree normalization excel in capturing local information, rendering Graph Neural Networks (GNNs) well-suited for tasks reliant on local connectivity. Nevertheless, the advantages of GSOs rooted in degree normalization may not extend seamlessly to all scenarios, particularly those demanding consideration of non-local information. In our study, we empirically highlight the constraints of traditional GSOs. To address these limitations, we introduce \textit{CGSO}, a novel class Graph Shift Operators. Unlike classical GSOs, \textit{CGSO} leverages global centrality metrics, such as PageRank score, $k$-core number, and the count of walks of a fixed length. This approach aims to enhance the adaptability of shift operators, making them more efficient in scenarios where non-local information is crucial.


